Conditional Generative Moment-Matching Networks

Maximum mean discrepancy (MMD) has been successfully applied to learn deep generative models for characterizing a joint distribution of variables via kernel mean embedding. In this paper, we present conditional generative moment- matching networks (CGMMN), which learn a conditional distribution given some input variables based on a conditional maximum mean discrepancy (CMMD) criterion. The learning is performed by stochastic gradient descent with the gradient calculated by back-propagation. We evaluate CGMMN on a wide range of tasks, including predictive modeling, contextual generation, and Bayesian dark knowledge, which distills knowledge from a Bayesian model by learning a relatively small CGMMN student network. Our results demonstrate competitive performance in all the tasks.

==> Makefile <==
TARGET=report
TEX=xelatex -shell-escape
BIBTEX=bibtex 
READER=evince

all: view

rebuild  output/$(TARGET).pdf: *.tex *.bib output
	cp *.sty output/ && cp -r images output/  && cd output && rm -f *.tex *.bib && ln -s ../*.tex ../*.bib .
	cd output && $(TEX) $(TARGET).tex && $(BIBTEX)$ $(TARGET).aux && \
		$(TEX) $(TARGET).tex  && $(TEX) $(TARGET).tex
	make

output: 
	mkdir output
	cd output && rm -f data src && ln -s ../data ../src .

view: output/$(TARGET).pdf
#	$(READER) output/$(TARGET).pdf &

clean:
	rm -rf output

.PHONY: all view clean rebuild dist

